Fictitious Cross-Play: Learning Global Nash Equilibrium in Mixed Cooperative-Competitive Games

Self-play (SP) is a popular multi-agent reinforcement learning (MARL) framework for solving competitive games, where each agent optimizes policy by treating others as part of the environment. Despite the empirical successes, the theoretical properties of SP-based methods are limited to two-player zero-sum games. However, for mixed cooperative-competitive games where agents on the same team need to cooperate with each other, we can show a simple counter-example where SP-based methods cannot converge to a global Nash equilibrium (NE) with high probability. Alternatively, Policy-Space Response Oracles (PSRO) is an iterative framework for learning NE, where the best responses w.r.t. previous policies are learned in each iteration. PSRO can be directly extended to mixed cooperative-competitive settings by jointly learning team best responses with all convergence properties unchanged. However, PSRO requires repeatedly training joint policies from scratch till convergence, which makes it hard to scale to complex games. In this work, we develop a novel algorithm, Fictitious Cross-Play (FXP), which inherits the benefits from both frameworks. FXP simultaneously trains an SP-based main policy and a counter population of best response policies. The main policy is trained by fictitious self-play and cross-play against the counter population, while the counter policies are trained as the best responses to the main policy's past versions. We validate our method in matrix games and show that FXP converges to global NEs while SP methods fail. We also conduct experiments in a gridworld domain, where FXP achieves higher Elo ratings and lower exploitabilities than baselines, and a more challenging football game, where FXP defeats SOTA models with over 94% win rate.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> reference.tex <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{36}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[\protect\citeauthoryear{Baker, Kanitscheider, Markov, Wu, Powell,
  McGrew, and Mordatch}{Baker et~al\mbox{.}}{2019}]%
        {baker2019emergent}
\bibfield{author}{\bibinfo{person}{Bowen Baker}, \bibinfo{person}{Ingmar
  Kanitscheider}, \bibinfo{person}{Todor Markov}, \bibinfo{person}{Yi Wu},
  \bibinfo{person}{Glenn Powell}, \bibinfo{person}{Bob McGrew}, {and}
  \bibinfo{person}{Igor Mordatch}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Emergent tool use from multi-agent autocurricula}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1909.07528}}
  (\bibinfo{year}{2019}).
\newblock


\bibitem[\protect\citeauthoryear{Balduzzi, Garnelo, Bachrach, Czarnecki,
  Perolat, Jaderberg, and Graepel}{Balduzzi et~al\mbox{.}}{2019}]%
        {balduzzi2019open}
\bibfield{author}{\bibinfo{person}{David Balduzzi}, \bibinfo{person}{Marta
  Garnelo}, \bibinfo{person}{Yoram Bachrach}, \bibinfo{person}{Wojciech
  Czarnecki}, \bibinfo{person}{Julien Perolat}, \bibinfo{person}{Max
  Jaderberg}, {and} \bibinfo{person}{Thore Graepel}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Open-ended learning in symmetric zero-sum games}.
  In \bibinfo{booktitle}{\emph{International Conference on Machine Learning}}.
  PMLR, \bibinfo{pages}{434--443}.
\newblock


\bibitem[\protect\citeauthoryear{Bansal, Pachocki, Sidor, Sutskever, and
  Mordatch}{Bansal et~al\mbox{.}}{2017}]%
        {bansal2017emergent}
\bibfield{author}{\bibinfo{person}{Trapit Bansal}, \bibinfo{person}{Jakub
  Pachocki}, \bibinfo{person}{Szymon Sidor}, \bibinfo{person}{Ilya Sutskever},
  {and} \bibinfo{person}{Igor Mordatch}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Emergent complexity via multi-agent competition}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1710.03748}}
  (\bibinfo{year}{2017}).
\newblock


\bibitem[\protect\citeauthoryear{Bard, Foerster, Chandar, Burch, Lanctot, Song,
  Parisotto, Dumoulin, Moitra, Hughes, et~al\mbox{.}}{Bard
  et~al\mbox{.}}{2020}]%
        {bard2020hanabi}
\bibfield{author}{\bibinfo{person}{Nolan Bard}, \bibinfo{person}{Jakob~N
  Foerster}, \bibinfo{person}{Sarath Chandar}, \bibinfo{person}{Neil Burch},
  \bibinfo{person}{Marc Lanctot}, \bibinfo{person}{H~Francis Song},
  \bibinfo{person}{Emilio Parisotto}, \bibinfo{person}{Vincent Dumoulin},
  \bibinfo{person}{Subhodeep Moitra}, \bibinfo{person}{Edward Hughes},
  {et~al\mbox{.}}} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{The hanabi challenge: A new frontier for ai
  research}.
\newblock \bibinfo{journal}{\emph{Artificial Intelligence}}
  \bibinfo{volume}{280} (\bibinfo{year}{2020}), \bibinfo{pages}{103216}.
\newblock


\bibitem[\protect\citeauthoryear{Berner, Brockman, Chan, Cheung, D{\k{e}}biak,
  Dennison, Farhi, Fischer, Hashme, Hesse, et~al\mbox{.}}{Berner
  et~al\mbox{.}}{2019}]%
        {berner2019dota}
\bibfield{author}{\bibinfo{person}{Christopher Berner}, \bibinfo{person}{Greg
  Brockman}, \bibinfo{person}{Brooke Chan}, \bibinfo{person}{Vicki Cheung},
  \bibinfo{person}{Przemys{\l}aw D{\k{e}}biak}, \bibinfo{person}{Christy
  Dennison}, \bibinfo{person}{David Farhi}, \bibinfo{person}{Quirin Fischer},
  \bibinfo{person}{Shariq Hashme}, \bibinfo{person}{Chris Hesse},
  {et~al\mbox{.}}} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Dota 2 with large scale deep reinforcement
  learning}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1912.06680}}
  (\bibinfo{year}{2019}).
\newblock


\bibitem[\protect\citeauthoryear{Blum and Monsour}{Blum and Monsour}{2007}]%
        {blum2007learning}
\bibfield{author}{\bibinfo{person}{Avrim Blum} {and} \bibinfo{person}{Yishay
  Monsour}.} \bibinfo{year}{2007}\natexlab{}.
\newblock \showarticletitle{Learning, regret minimization, and equilibria}.
\newblock  (\bibinfo{year}{2007}).
\newblock


\bibitem[\protect\citeauthoryear{Brown}{Brown}{1951}]%
        {brown1951iterative}
\bibfield{author}{\bibinfo{person}{George~W Brown}.}
  \bibinfo{year}{1951}\natexlab{}.
\newblock \showarticletitle{Iterative solution of games by fictitious play}.
\newblock \bibinfo{journal}{\emph{Act. Anal. Prod Allocation}}
  \bibinfo{volume}{13}, \bibinfo{number}{1} (\bibinfo{year}{1951}),
  \bibinfo{pages}{374}.
\newblock


\bibitem[\protect\citeauthoryear{Brown, Lerer, Gross, and Sandholm}{Brown
  et~al\mbox{.}}{2019}]%
        {brown2019deep}
\bibfield{author}{\bibinfo{person}{Noam Brown}, \bibinfo{person}{Adam Lerer},
  \bibinfo{person}{Sam Gross}, {and} \bibinfo{person}{Tuomas Sandholm}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Deep counterfactual regret minimization}. In
  \bibinfo{booktitle}{\emph{International conference on machine learning}}.
  PMLR, \bibinfo{pages}{793--802}.
\newblock


\bibitem[\protect\citeauthoryear{Dinh, Yang, Tian, Nieves, Slumbers, Mguni,
  Ammar, and Wang}{Dinh et~al\mbox{.}}{2021}]%
        {dinh2021online}
\bibfield{author}{\bibinfo{person}{Le~Cong Dinh}, \bibinfo{person}{Yaodong
  Yang}, \bibinfo{person}{Zheng Tian}, \bibinfo{person}{Nicolas~Perez Nieves},
  \bibinfo{person}{Oliver Slumbers}, \bibinfo{person}{David~Henry Mguni},
  \bibinfo{person}{Haitham~Bou Ammar}, {and} \bibinfo{person}{Jun Wang}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Online Double Oracle}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2103.07780}}
  (\bibinfo{year}{2021}).
\newblock


\bibitem[\protect\citeauthoryear{Elo}{Elo}{1978}]%
        {elo1978rating}
\bibfield{author}{\bibinfo{person}{Arpad~E Elo}.}
  \bibinfo{year}{1978}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{The rating of chessplayers, past and
  present}}.
\newblock \bibinfo{publisher}{Arco Pub.}
\newblock


\bibitem[\protect\citeauthoryear{Freund and Schapire}{Freund and
  Schapire}{1999}]%
        {freund1999adaptive}
\bibfield{author}{\bibinfo{person}{Yoav Freund} {and} \bibinfo{person}{Robert~E
  Schapire}.} \bibinfo{year}{1999}\natexlab{}.
\newblock \showarticletitle{Adaptive game playing using multiplicative
  weights}.
\newblock \bibinfo{journal}{\emph{Games and Economic Behavior}}
  \bibinfo{volume}{29}, \bibinfo{number}{1-2} (\bibinfo{year}{1999}),
  \bibinfo{pages}{79--103}.
\newblock


\bibitem[\protect\citeauthoryear{Heinrich, Lanctot, and Silver}{Heinrich
  et~al\mbox{.}}{2015}]%
        {heinrich2015fictitious}
\bibfield{author}{\bibinfo{person}{Johannes Heinrich}, \bibinfo{person}{Marc
  Lanctot}, {and} \bibinfo{person}{David Silver}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Fictitious self-play in extensive-form games}. In
  \bibinfo{booktitle}{\emph{International conference on machine learning}}.
  PMLR, \bibinfo{pages}{805--813}.
\newblock


\bibitem[\protect\citeauthoryear{Heinrich and Silver}{Heinrich and
  Silver}{2016}]%
        {heinrich2016deep}
\bibfield{author}{\bibinfo{person}{Johannes Heinrich} {and}
  \bibinfo{person}{David Silver}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Deep reinforcement learning from self-play in
  imperfect-information games}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1603.01121}}
  (\bibinfo{year}{2016}).
\newblock


\bibitem[\protect\citeauthoryear{Hennes, Morrill, Omidshafiei, Munos, Perolat,
  Lanctot, Gruslys, Lespiau, Parmas, Du{\'e}{\~n}ez-Guzm{\'a}n,
  et~al\mbox{.}}{Hennes et~al\mbox{.}}{2020}]%
        {hennes2020neural}
\bibfield{author}{\bibinfo{person}{Daniel Hennes}, \bibinfo{person}{Dustin
  Morrill}, \bibinfo{person}{Shayegan Omidshafiei}, \bibinfo{person}{R{\'e}mi
  Munos}, \bibinfo{person}{Julien Perolat}, \bibinfo{person}{Marc Lanctot},
  \bibinfo{person}{Audrunas Gruslys}, \bibinfo{person}{Jean-Baptiste Lespiau},
  \bibinfo{person}{Paavo Parmas}, \bibinfo{person}{Edgar
  Du{\'e}{\~n}ez-Guzm{\'a}n}, {et~al\mbox{.}}} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Neural replicator dynamics: Multiagent learning via
  hedging policy gradients}. In \bibinfo{booktitle}{\emph{Proceedings of the
  19th International Conference on Autonomous Agents and MultiAgent Systems}}.
  \bibinfo{pages}{492--501}.
\newblock


\bibitem[\protect\citeauthoryear{Huang, Chen, Zhang, Li, Zhu, Ye, Chen, and
  Zhu}{Huang et~al\mbox{.}}{2021}]%
        {huang2021tikick}
\bibfield{author}{\bibinfo{person}{Shiyu Huang}, \bibinfo{person}{Wenze Chen},
  \bibinfo{person}{Longfei Zhang}, \bibinfo{person}{Ziyang Li},
  \bibinfo{person}{Fengming Zhu}, \bibinfo{person}{Deheng Ye},
  \bibinfo{person}{Ting Chen}, {and} \bibinfo{person}{Jun Zhu}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{TiKick: Towards Playing Multi-agent Football Full
  Games from Single-agent Demonstrations}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2110.04507}}
  (\bibinfo{year}{2021}).
\newblock


\bibitem[\protect\citeauthoryear{Jaderberg, Czarnecki, Dunning, Marris, Lever,
  Castaneda, Beattie, Rabinowitz, Morcos, Ruderman, et~al\mbox{.}}{Jaderberg
  et~al\mbox{.}}{2019}]%
        {jaderberg2019human}
\bibfield{author}{\bibinfo{person}{Max Jaderberg}, \bibinfo{person}{Wojciech~M
  Czarnecki}, \bibinfo{person}{Iain Dunning}, \bibinfo{person}{Luke Marris},
  \bibinfo{person}{Guy Lever}, \bibinfo{person}{Antonio~Garcia Castaneda},
  \bibinfo{person}{Charles Beattie}, \bibinfo{person}{Neil~C Rabinowitz},
  \bibinfo{person}{Ari~S Morcos}, \bibinfo{person}{Avraham Ruderman},
  {et~al\mbox{.}}} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Human-level performance in 3D multiplayer games
  with population-based reinforcement learning}.
\newblock \bibinfo{journal}{\emph{Science}} \bibinfo{volume}{364},
  \bibinfo{number}{6443} (\bibinfo{year}{2019}), \bibinfo{pages}{859--865}.
\newblock


\bibitem[\protect\citeauthoryear{Kurach, Raichuk, Sta{\'n}czyk, Zaj{\k{a}}c,
  Bachem, Espeholt, Riquelme, Vincent, Michalski, Bousquet,
  et~al\mbox{.}}{Kurach et~al\mbox{.}}{2020}]%
        {kurach2020google}
\bibfield{author}{\bibinfo{person}{Karol Kurach}, \bibinfo{person}{Anton
  Raichuk}, \bibinfo{person}{Piotr Sta{\'n}czyk}, \bibinfo{person}{Micha{\l}
  Zaj{\k{a}}c}, \bibinfo{person}{Olivier Bachem}, \bibinfo{person}{Lasse
  Espeholt}, \bibinfo{person}{Carlos Riquelme}, \bibinfo{person}{Damien
  Vincent}, \bibinfo{person}{Marcin Michalski}, \bibinfo{person}{Olivier
  Bousquet}, {et~al\mbox{.}}} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Google research football: A novel reinforcement
  learning environment}. In \bibinfo{booktitle}{\emph{Proceedings of the AAAI
  Conference on Artificial Intelligence}}, Vol.~\bibinfo{volume}{34}.
  \bibinfo{pages}{4501--4510}.
\newblock


\bibitem[\protect\citeauthoryear{Lanctot, Zambaldi, Gruslys, Lazaridou, Tuyls,
  P{\'e}rolat, Silver, and Graepel}{Lanctot et~al\mbox{.}}{2017}]%
        {lanctot2017unified}
\bibfield{author}{\bibinfo{person}{Marc Lanctot}, \bibinfo{person}{Vinicius
  Zambaldi}, \bibinfo{person}{Audrunas Gruslys}, \bibinfo{person}{Angeliki
  Lazaridou}, \bibinfo{person}{Karl Tuyls}, \bibinfo{person}{Julien
  P{\'e}rolat}, \bibinfo{person}{David Silver}, {and} \bibinfo{person}{Thore
  Graepel}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{A unified game-theoretic approach to multiagent
  reinforcement learning}.
\newblock \bibinfo{journal}{\emph{Advances in neural information processing
  systems}}  \bibinfo{volume}{30} (\bibinfo{year}{2017}).
\newblock


\bibitem[\protect\citeauthoryear{Littman}{Littman}{1994}]%
        {littman1994markov}
\bibfield{author}{\bibinfo{person}{Michael~L Littman}.}
  \bibinfo{year}{1994}\natexlab{}.
\newblock \showarticletitle{Markov games as a framework for multi-agent
  reinforcement learning}. In \bibinfo{booktitle}{\emph{Proceedings of the
  eleventh international conference on machine learning}},
  Vol.~\bibinfo{volume}{157}. \bibinfo{pages}{157--163}.
\newblock


\bibitem[\protect\citeauthoryear{Liu, Jia, Wen, Hu, Chen, Fan, Hu, and
  Yang}{Liu et~al\mbox{.}}{2021}]%
        {liu2021towards}
\bibfield{author}{\bibinfo{person}{Xiangyu Liu}, \bibinfo{person}{Hangtian
  Jia}, \bibinfo{person}{Ying Wen}, \bibinfo{person}{Yujing Hu},
  \bibinfo{person}{Yingfeng Chen}, \bibinfo{person}{Changjie Fan},
  \bibinfo{person}{Zhipeng Hu}, {and} \bibinfo{person}{Yaodong Yang}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Towards Unifying Behavioral and Response Diversity
  for Open-ended Learning in Zero-sum Games}.
\newblock \bibinfo{journal}{\emph{Advances in Neural Information Processing
  Systems}}  \bibinfo{volume}{34} (\bibinfo{year}{2021}),
  \bibinfo{pages}{941--952}.
\newblock


\bibitem[\protect\citeauthoryear{Lowe, Wu, Tamar, Harb, Pieter~Abbeel, and
  Mordatch}{Lowe et~al\mbox{.}}{2017}]%
        {lowe2017multi}
\bibfield{author}{\bibinfo{person}{Ryan Lowe}, \bibinfo{person}{Yi~I Wu},
  \bibinfo{person}{Aviv Tamar}, \bibinfo{person}{Jean Harb},
  \bibinfo{person}{OpenAI Pieter~Abbeel}, {and} \bibinfo{person}{Igor
  Mordatch}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Multi-agent actor-critic for mixed
  cooperative-competitive environments}.
\newblock \bibinfo{journal}{\emph{Advances in neural information processing
  systems}}  \bibinfo{volume}{30} (\bibinfo{year}{2017}).
\newblock


\bibitem[\protect\citeauthoryear{McAleer, Lanier, Wang, Baldi, and Fox}{McAleer
  et~al\mbox{.}}{2021}]%
        {mcaleer2021xdo}
\bibfield{author}{\bibinfo{person}{Stephen McAleer}, \bibinfo{person}{John~B
  Lanier}, \bibinfo{person}{Kevin~A Wang}, \bibinfo{person}{Pierre Baldi},
  {and} \bibinfo{person}{Roy Fox}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{XDO: A double oracle algorithm for extensive-form
  games}.
\newblock \bibinfo{journal}{\emph{Advances in Neural Information Processing
  Systems}}  \bibinfo{volume}{34} (\bibinfo{year}{2021}),
  \bibinfo{pages}{23128--23139}.
\newblock


\bibitem[\protect\citeauthoryear{McAleer, Wang, Lanier, Lanctot, Baldi,
  Sandholm, and Fox}{McAleer et~al\mbox{.}}{2022}]%
        {mcaleer2022anytime}
\bibfield{author}{\bibinfo{person}{Stephen McAleer}, \bibinfo{person}{Kevin
  Wang}, \bibinfo{person}{JB Lanier}, \bibinfo{person}{Marc Lanctot},
  \bibinfo{person}{Pierre Baldi}, \bibinfo{person}{Tuomas Sandholm}, {and}
  \bibinfo{person}{Roy Fox}.} \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{Anytime PSRO for Two-Player Zero-Sum Games}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2201.07700}}
  (\bibinfo{year}{2022}).
\newblock


\bibitem[\protect\citeauthoryear{McMahan, Gordon, and Blum}{McMahan
  et~al\mbox{.}}{2003}]%
        {mcmahan2003planning}
\bibfield{author}{\bibinfo{person}{H~Brendan McMahan},
  \bibinfo{person}{Geoffrey~J Gordon}, {and} \bibinfo{person}{Avrim Blum}.}
  \bibinfo{year}{2003}\natexlab{}.
\newblock \showarticletitle{Planning in the presence of cost functions
  controlled by an adversary}. In \bibinfo{booktitle}{\emph{Proceedings of the
  20th International Conference on Machine Learning (ICML-03)}}.
  \bibinfo{pages}{536--543}.
\newblock


\bibitem[\protect\citeauthoryear{Muller, Omidshafiei, Rowland, Tuyls, Perolat,
  Liu, Hennes, Marris, Lanctot, Hughes, et~al\mbox{.}}{Muller
  et~al\mbox{.}}{2019}]%
        {muller2019generalized}
\bibfield{author}{\bibinfo{person}{Paul Muller}, \bibinfo{person}{Shayegan
  Omidshafiei}, \bibinfo{person}{Mark Rowland}, \bibinfo{person}{Karl Tuyls},
  \bibinfo{person}{Julien Perolat}, \bibinfo{person}{Siqi Liu},
  \bibinfo{person}{Daniel Hennes}, \bibinfo{person}{Luke Marris},
  \bibinfo{person}{Marc Lanctot}, \bibinfo{person}{Edward Hughes},
  {et~al\mbox{.}}} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{A generalized training approach for multiagent
  learning}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1909.12823}}
  (\bibinfo{year}{2019}).
\newblock


\bibitem[\protect\citeauthoryear{Perez-Nieves, Yang, Slumbers, Mguni, Wen, and
  Wang}{Perez-Nieves et~al\mbox{.}}{2021}]%
        {perez2021modelling}
\bibfield{author}{\bibinfo{person}{Nicolas Perez-Nieves},
  \bibinfo{person}{Yaodong Yang}, \bibinfo{person}{Oliver Slumbers},
  \bibinfo{person}{David~H Mguni}, \bibinfo{person}{Ying Wen}, {and}
  \bibinfo{person}{Jun Wang}.} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{Modelling behavioural diversity for learning in
  open-ended games}. In \bibinfo{booktitle}{\emph{International Conference on
  Machine Learning}}. PMLR, \bibinfo{pages}{8514--8524}.
\newblock


\bibitem[\protect\citeauthoryear{Perolat, Munos, Lespiau, Omidshafiei, Rowland,
  Ortega, Burch, Anthony, Balduzzi, De~Vylder, et~al\mbox{.}}{Perolat
  et~al\mbox{.}}{2021}]%
        {perolat2021poincare}
\bibfield{author}{\bibinfo{person}{Julien Perolat}, \bibinfo{person}{Remi
  Munos}, \bibinfo{person}{Jean-Baptiste Lespiau}, \bibinfo{person}{Shayegan
  Omidshafiei}, \bibinfo{person}{Mark Rowland}, \bibinfo{person}{Pedro Ortega},
  \bibinfo{person}{Neil Burch}, \bibinfo{person}{Thomas Anthony},
  \bibinfo{person}{David Balduzzi}, \bibinfo{person}{Bart De~Vylder},
  {et~al\mbox{.}}} \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{From Poincar{\'e} recurrence to convergence in
  imperfect information games: Finding equilibrium via regularization}. In
  \bibinfo{booktitle}{\emph{International Conference on Machine Learning}}.
  PMLR, \bibinfo{pages}{8525--8535}.
\newblock


\bibitem[\protect\citeauthoryear{Rashid, Samvelyan, Schroeder, Farquhar,
  Foerster, and Whiteson}{Rashid et~al\mbox{.}}{2018}]%
        {rashid2018qmix}
\bibfield{author}{\bibinfo{person}{Tabish Rashid}, \bibinfo{person}{Mikayel
  Samvelyan}, \bibinfo{person}{Christian Schroeder}, \bibinfo{person}{Gregory
  Farquhar}, \bibinfo{person}{Jakob Foerster}, {and} \bibinfo{person}{Shimon
  Whiteson}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Qmix: Monotonic value function factorisation for
  deep multi-agent reinforcement learning}. In
  \bibinfo{booktitle}{\emph{International conference on machine learning}}.
  PMLR, \bibinfo{pages}{4295--4304}.
\newblock


\bibitem[\protect\citeauthoryear{Ratliff, Burden, and Sastry}{Ratliff
  et~al\mbox{.}}{2013}]%
        {ratliff2013characterization}
\bibfield{author}{\bibinfo{person}{Lillian~J Ratliff},
  \bibinfo{person}{Samuel~A Burden}, {and} \bibinfo{person}{S~Shankar Sastry}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Characterization and computation of local Nash
  equilibria in continuous games}. In \bibinfo{booktitle}{\emph{2013 51st
  Annual Allerton Conference on Communication, Control, and Computing
  (Allerton)}}. IEEE, \bibinfo{pages}{917--924}.
\newblock


\bibitem[\protect\citeauthoryear{Shalev-Shwartz et~al\mbox{.}}{Shalev-Shwartz
  et~al\mbox{.}}{2012}]%
        {shalev2012online}
\bibfield{author}{\bibinfo{person}{Shai Shalev-Shwartz} {et~al\mbox{.}}}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Online learning and online convex optimization}.
\newblock \bibinfo{journal}{\emph{Foundations and Trends{\textregistered} in
  Machine Learning}} \bibinfo{volume}{4}, \bibinfo{number}{2}
  (\bibinfo{year}{2012}), \bibinfo{pages}{107--194}.
\newblock


\bibitem[\protect\citeauthoryear{Silver, Huang, Maddison, Guez, Sifre, Van
  Den~Driessche, Schrittwieser, Antonoglou, Panneershelvam, Lanctot,
  et~al\mbox{.}}{Silver et~al\mbox{.}}{2016}]%
        {silver2016mastering}
\bibfield{author}{\bibinfo{person}{David Silver}, \bibinfo{person}{Aja Huang},
  \bibinfo{person}{Chris~J Maddison}, \bibinfo{person}{Arthur Guez},
  \bibinfo{person}{Laurent Sifre}, \bibinfo{person}{George Van Den~Driessche},
  \bibinfo{person}{Julian Schrittwieser}, \bibinfo{person}{Ioannis Antonoglou},
  \bibinfo{person}{Veda Panneershelvam}, \bibinfo{person}{Marc Lanctot},
  {et~al\mbox{.}}} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Mastering the game of Go with deep neural networks
  and tree search}.
\newblock \bibinfo{journal}{\emph{nature}} \bibinfo{volume}{529},
  \bibinfo{number}{7587} (\bibinfo{year}{2016}), \bibinfo{pages}{484--489}.
\newblock


\bibitem[\protect\citeauthoryear{Sokota, D'Orazio, Kolter, Loizou, Lanctot,
  Mitliagkas, Brown, and Kroer}{Sokota et~al\mbox{.}}{2022}]%
        {sokota2022unified}
\bibfield{author}{\bibinfo{person}{Samuel Sokota}, \bibinfo{person}{Ryan
  D'Orazio}, \bibinfo{person}{J~Zico Kolter}, \bibinfo{person}{Nicolas Loizou},
  \bibinfo{person}{Marc Lanctot}, \bibinfo{person}{Ioannis Mitliagkas},
  \bibinfo{person}{Noam Brown}, {and} \bibinfo{person}{Christian Kroer}.}
  \bibinfo{year}{2022}\natexlab{}.
\newblock \showarticletitle{A unified approach to reinforcement learning,
  quantal response equilibria, and two-player zero-sum games}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2206.05825}}
  (\bibinfo{year}{2022}).
\newblock


\bibitem[\protect\citeauthoryear{Tesauro}{Tesauro}{1994}]%
        {tesauro1994td}
\bibfield{author}{\bibinfo{person}{Gerald Tesauro}.}
  \bibinfo{year}{1994}\natexlab{}.
\newblock \showarticletitle{TD-Gammon, a self-teaching backgammon program,
  achieves master-level play}.
\newblock \bibinfo{journal}{\emph{Neural computation}} \bibinfo{volume}{6},
  \bibinfo{number}{2} (\bibinfo{year}{1994}), \bibinfo{pages}{215--219}.
\newblock


\bibitem[\protect\citeauthoryear{Vinyals, Babuschkin, Czarnecki, Mathieu,
  Dudzik, Chung, Choi, Powell, Ewalds, Georgiev, et~al\mbox{.}}{Vinyals
  et~al\mbox{.}}{2019}]%
        {vinyals2019grandmaster}
\bibfield{author}{\bibinfo{person}{Oriol Vinyals}, \bibinfo{person}{Igor
  Babuschkin}, \bibinfo{person}{Wojciech~M Czarnecki},
  \bibinfo{person}{Micha{\"e}l Mathieu}, \bibinfo{person}{Andrew Dudzik},
  \bibinfo{person}{Junyoung Chung}, \bibinfo{person}{David~H Choi},
  \bibinfo{person}{Richard Powell}, \bibinfo{person}{Timo Ewalds},
  \bibinfo{person}{Petko Georgiev}, {et~al\mbox{.}}}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Grandmaster level in StarCraft II using multi-agent
  reinforcement learning}.
\newblock \bibinfo{journal}{\emph{Nature}} \bibinfo{volume}{575},
  \bibinfo{number}{7782} (\bibinfo{year}{2019}), \bibinfo{pages}{350--354}.
\newblock


\bibitem[\protect\citeauthoryear{Yu, Velu, Vinitsky, Wang, Bayen, and Wu}{Yu
  et~al\mbox{.}}{2021}]%
        {yu2021surprising}
\bibfield{author}{\bibinfo{person}{Chao Yu}, \bibinfo{person}{Akash Velu},
  \bibinfo{person}{Eugene Vinitsky}, \bibinfo{person}{Yu Wang},
  \bibinfo{person}{Alexandre Bayen}, {and} \bibinfo{person}{Yi Wu}.}
  \bibinfo{year}{2021}\natexlab{}.
\newblock \showarticletitle{The surprising effectiveness of ppo in cooperative,
  multi-agent games}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2103.01955}}
  (\bibinfo{year}{2021}).
\newblock


\bibitem[\protect\citeauthoryear{Zheng, Yang, Cai, Zhou, Zhang, Wang, and
  Yu}{Zheng et~al\mbox{.}}{2018}]%
        {zheng2018magent}
\bibfield{author}{\bibinfo{person}{Lianmin Zheng}, \bibinfo{person}{Jiacheng
  Yang}, \bibinfo{person}{Han Cai}, \bibinfo{person}{Ming Zhou},
  \bibinfo{person}{Weinan Zhang}, \bibinfo{person}{Jun Wang}, {and}
  \bibinfo{person}{Yong Yu}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Magent: A many-agent reinforcement learning
  platform for artificial collective intelligence}. In
  \bibinfo{booktitle}{\emph{Proceedings of the AAAI conference on artificial
  intelligence}}, Vol.~\bibinfo{volume}{32}.
\newblock


\end{thebibliography}

